Analytical energy gradient for state-averaged orbital-optimized variational quantum eigensolvers and its application to a photochemical reaction

Elucidating photochemical reactions is vital to understand various biochemical phenomena and develop functional materials such as artificial photosynthesis and organic solar cells, albeit its notorious difficulty by both experiments and theories. The best theoretical way so far to analyze photochemical reactions at the level of ab initio electronic structure is the state-averaged multi-configurational self-consistent field (SA-MCSCF) method. However, the exponential computational cost of classical computers with the increasing number of molecular orbitals hinders applications of SA-MCSCF for large systems we are interested in. Utilizing quantum computers was recently proposed as a promising approach to overcome such computational cost, dubbed as state-averaged orbital-optimized variational quantum eigensolver (SA-OO-VQE). Here we extend a theory of SA-OO-VQE so that analytical gradients of energy can be evaluated by standard techniques that are feasible with near-term quantum computers. The analytical gradients, known only for the state-specific OO-VQE in previous studies, allow us to determine various characteristics of photochemical reactions such as the conical intersection (CI) points. We perform a proof-of-principle calculation of our methods by applying it to the photochemical cis-trans isomerization of 1,3,3,3-tetrafluoropropene. Numerical simulations of quantum circuits and measurements can correctly capture the photochemical reaction pathway of this model system, including the CI points. Our results illustrate the possibility of leveraging quantum computers for studying photochemical reactions.

==> disucussion_old.tex <==
\section{Discussion}
\subsection{\label{subsec:estimation}Estimation of the number of circuits}
In this section, we estimate the number of circuits to be measured for evaluating analytical gradients in addition to circuits to determine the optimized wavefunction. We assume one- and two-body reduced density matrix (1-RDMs and 2-RDMs, respectively) at the optimal values are already measured. To calculate the analytical gradient, we need to solve the linear equation in Eq.\eqref{eq:linear equation vqd}. Therefore $\mathbb{H}^{\rm{VV,VO,OV,OO}}$ and $\bm{g}^A$ need to be measured. 

We assume that the number of gates in $\hat{U}(\bm{\theta})$ is denoted as $d$, which means that the ansatz circuit is a sequence of $d$ Pauli rotations, and the number of states under consideration is $K$. 
\begin{comment}
\subsubsection{The number of additional circuits for SA-OO-SSVQE}
In SA-OO-SSVQE, we assume that RDMs at the optimal values such as $\bra{\psi_S}\hat{U}^\dag(\bm{\theta}^*)\hat{a}_{p\sigma}^\dag\hat{a}_{q\sigma}\hat{U}(\bm{\theta}^*)\ket{\psi_S}\,\,(S=1\sim K)$ are already obtained. To calculate the analytical gradient in Eq.\eqref{eq:inter_expression}, we need to solve the linear equation in Eq.\eqref{matrix_eqs}. Therefore, $\mathbb{H}^{\rm{VV,VO,OV,OO}}, \bm{f}^A$, and $\bm{g}^A$ need to be measured:
\begin{itemize}
    \item $\mathbb{H}^{\rm{VV}}$ is obtained by ``parameter shift rule" in a way described in Sec.\ref{subsec:circuit derivative}. Diagonal elements $\partial^2E^{\rm{SSVQE}}/\partial\theta_i^2$ require 2 new circuits and non-diagonal elements $\partial^2E^{\rm{SSVQE}}/\partial\theta_i\partial\theta_j\,\,(i\not=j)$ require 4 new circuits. Therefore, in total we need ${d\choose 2}\times 4+d\times 2=2d^2$ additional circuit.
    \item $\mathbb{H}^{\rm{VO}}$ is also obtained by parameter shift rule. Since only first-order derivatives with respect to the circuit parameters are involved, for each $\partial^2E^{\rm{SSVQE}}/\partial\theta_i\partial\kappa_{pq}$ with $\forall p,q$, 2 additional circuits are required. Therefore in total we need $2d$ new circuits.
    \item $\mathbb{H}^{\rm{OV}}$ and $\bm{f}^A$ do not require any new circuit since parameters-shifted circuits corresponding to first-order derivatives are already prepared in calculating $\mathbb{H}^{\rm{VO}}$.
    \end{itemize}
Note that $\bm{\kappa}$ derivative does not require new circuits since as discussed in Sec.\ref{subsec:orbital derivative}, it is replaced by the commutator, which is a sum of RDMs at given circuit parameters.   

In total, we need $2d(d+1)$ additional circuits.
\end{comment}
%To do so, the derivative with respect to the orbital parameters $\bm{\kappa}$ and the circuit parameters $\bm{\theta}$ are required. The $\bm{\kappa}$ derivative does not require any new circuits since it is just a commutator at optimal values, being a sum of 1-RDMs and 2-RDMs. The $\bm{\theta}$ derivative requires new circuits due to the parameter shift rule in Eq.(\ref{eq:theta derivative}). Terms which involve the first derivative in $\bm{\theta}$, such as $\bm{f}$ in Eq.(\ref{eq:vqe matrix}) requires $2d$ new circuits and $\mathbb{H}^{\mr{VV}}$ which the second derivative is necessary to evaluate requires $2d^2$ circuits. Therefore for each level we need to construct $2d(d+1)$ circuits in addition to those for the optimization.

%\subsubsection{The number of additional circuits for SA-OO-VQD}
%In SA-OO-VQD, the procedures are essentially the same as SA-OO-SSVQE. Therefore we need to enumerate the number of the parameter shifted circuits in evaluating $\mathbb{H}^{\rm{VV, VO, OV, OO}}$. However, the overlap term in the definition of $F_S^{\rm{VQD}}$ adds another complication.
\begin{itemize}
    \item We split $\mathbb{H}^{\rm{VV}}$ into ``diagonal blocks", i.e., $\mathbb{H}^{\rm{VV}}_{(Si)(Sj)}$ and non-diagonal blocks. For each diagonal block, each element $\partial^2F_S^{\rm{VQD}}/\partial\theta_{Si}\partial\theta_{Sj}$ requires $2d^2$ additional circuits due to ``parameter shift rule". In total, diagonal blocks require $2d^2K$ circuits. For non-diagonal blocks, $\mathbb{H}^{\rm{VV}}$ amounts to the second-order derivative of a sum of overlaps: when $T<S$, its element is
    \begin{equation}\label{eq:derivative overlap}\begin{aligned}
        \mathbb{H}^{\rm{VV}}_{(Tj)(Si)}&=\beta_T\Bigg(\bra{\psi}\hat{U}^\dag(\bm{\theta_S})\left(\pdv{\hat{U}(\bm{\theta}_T)}{\theta_{Tj}}\right)\ket{\psi}\bra{\psi}\hat{U}^\dag(\bm{\theta}_T)\left(\pdv{\hat{U}(\bm{\theta}_S)}{\theta_{Si}}\right)\ket{\psi}+c.c.\Bigg),
        \end{aligned}
    \end{equation}
    where $c.c.$ means taking complex conjugate and we make use of the fact that the overlap at the optimal values should be zero. Eq.\eqref{eq:derivative overlap} requires 2 additional circuits. Therefore, for each non-diagonal block there are $2d^2$ circuits necessary. In total, for evaluating $\mathbb{H}^{\rm{VV}}$ in non-diagonal blocks we need $\binom{K}{2}\times 2d^2=d^2K(K-1)$ additional circuits.
    
    Combining diagonal and non-diagonal parts together yields $2d^2K+d^2K(K-1)=d^2K(K+1)$ new circuits.
    \item $\mathbb{H}^{\rm{VO}}$ is also obtained by parameter shift rule. As only first-order derivatives with respect to circuit parameters are involved, for each $\mathbb{H}^{\rm{VO}}_{(Tj)(pq)}$ with $\forall p,q$, 2 additional circuits are required. Therefore we need $2dK$ circuits.
    \item $\mathbb{H}^{\rm{OV}}, \mathbb{H}^{\rm{OO}},$ and $\bm{g}^A$ do not require new circuits as at most first-order derivatives with respect to circuit parameters are involved and they are already measured to evaluate $\mathbb{H}^{\rm{VO}}$. 
    \end{itemize}
In total, the number of new circuits for SA-OO-VQD is $dK(d(K+1)+2)$.

\begin{comment}
\subsubsection{The number of additional circuits for SA-OO-MCVQE}
In SA-OO-MCVQE, we also need to enumerate the number of the parameter shifted circuits in Hessian matrices $\mathbb{H}^{\rm{VV, VO, OV, OO}}$ and vectors $\bm{f}^{ST}$. Since the only difference between SA-OO-MCVQE and SA-OO-SSVQE is that we consider non-diagonal elements, i.e., $\bra{\psi_S}\hat{U}^\dag(\bm{\theta})\hat{\mathcal{H}}(\bm{x},\bm{\kappa})\hat{U}(\bm{\theta})\ket{\psi_T}$ in SA-OO-MCVQE while we do not consider them in SA-OO-SSVQE. This difference leads to different definition of vectors $\bm{f}^{ST}$ and $\bm{g}^{ST}$, which does not affect the number of additionally required circuits. Therefore the number of new circuits is $2d(d+1)$. 
\end{comment}

\begin{comment}
\subsection{Comparison with the straightforward calculation}
To appreciate advantages of the Lagrangian method we have developed, we compare it to the straightforward calculation. The gradient of the energy for the state $A$ is written as
\begin{equation}\begin{split}
    \dv{E^*_A(\bm{x})}{x_\mu}&=\bra{\psi}\hat{U}^\dag(\bm{\theta}_A^*)\pdv{\hat{H}(\bm{x},\bm{\kappa}^*)}{x_\mu}\hat{U}(\bm{\theta}_A^*)\ket{\psi}+\sum_i\dv{\theta^*_{Ai}}{x_\mu}\pdv{E_A(\bm{x},\bm{\theta}_A^*,\bm{\kappa}^*)}{\theta_{Ai}}\\&+\sum_{p>q}\dv{\kappa^*_{pq}}{x_\mu}\pdv{E_A(\bm{x},\bm{\theta}_A^*,\bm{\kappa}^*)}{\kappa_{pq}}.
    \end{split}
\end{equation}
Derivatives of parameters $d\bm{\theta}_A^*/dx_\mu$ and $d\bm{\kappa}^*/dx_\mu$ are calculated in the following way. Since $F_A^{\rm{VQD}}$ and $E^{\rm{SA}}$ are optimal with respect to $\bm{\theta}_A$ and $\bm{\kappa}$, respectively, we obtain
\begin{equation}
    \begin{split}
        &\dv{x_\mu}\left(\pdv{F_A^{\rm{VQD}}}{\theta_{Aj}}\right)=\pdv{\theta_j}\bra{\psi}\hat{U}^\dag(\bm{\theta}_A^*)\pdv{\hat{\mathcal{H}}(\bm{x},\bm{\kappa}^*)}{x_\mu}\hat{U}(\bm{\theta}_A^*)\ket{\psi}\\&+\sum_i\dv{\theta_{Ai}}{x_\mu}\pdv{E_A(\bm{x},\bm{\theta}_A^*,\bm{\kappa}^*)}{\theta_{Ai}}{\theta_{Aj}}+\sum_{p>q}\dv{\kappa_{pq}}{x_\mu}\pdv{E_A(\bm{x},\bm{\theta}_A^*,\bm{\kappa}^*)}{\kappa_{pq}}{\theta_{Aj}}=0\\
        &\dv{x_\mu}\left(\pdv{E^{\rm{SA}}}{\kappa_{rs}}\right)
        =\sum_S\omega_S^{\rm{SA}}\pdv{\kappa_{rs}}\bra{\psi}\hat{U}^\dag(\bm{\theta}_S^*)\pdv{\hat{\mathcal{H}}(\bm{x},\bm{\kappa}^*)}{x_\mu}\hat{U}(\bm{\theta}_S^*)\ket{\psi}\\
        &+\sum_{Si}\dv{\theta_{Si}}{x_\mu}\pdv{E^{\rm{SA}}}{\theta_{Si}}{\kappa_{rs}}+\sum_{p>q}\dv{\kappa_{pq}}{x_\mu}\pdv{E^{\rm{SA}}}{\kappa_{pq}}{\kappa_{rs}}=0.
    \end{split}
\end{equation}
This equation is also expressed in the following matrix form.
\begin{equation}\label{eq:straightforward linear}
    \begin{pmatrix}
    \left(\widetilde{\mathbb{H}}^{\rm{VV}}\right)^{\rm{T}}&\left(\mathbb{H}^{\rm{OV}}\right)^{\rm{T}}\\
    \left(\mathbb{H}^{\rm{VO}}\right)^{\rm{T}}&\left(\mathbb{H}^{\rm{OO}}\right)^{\mr{T}}
    \end{pmatrix}
    \begin{pmatrix}
    \dv{\bm{\theta}_0}{x_\mu}\\\vdots\\\dv{\bm{\theta}_{K-1}}{x_\mu}\\\dv{\bm{\kappa}}{x_\mu}
    \end{pmatrix}=-\begin{pmatrix}
    \pdv{E_0}{\bm{\theta}_0}{x_\mu}\\\vdots\\\pdv{E_{K-1}}{\bm{\theta}_{K-1}}{x_\mu}\\
    \pdv{E^{\rm{SA}}}{\bm{\kappa}}{x_\mu},
    \end{pmatrix}
\end{equation}
where $\widetilde{\mathbb{H}}^{\rm{VV}}$ is a ``diagonal part" of $\mathbb{H}^{\rm{VV}}$, i.e., $\widetilde{\mathbb{H}}^{\rm{VV}}_{(Tj)(Si)}=\delta_{ST}\mathbb{H}_{(Tj)(Si)}^{\rm{VV}}$ and 
\begin{equation}
    \begin{split}
        %&\pdv{E^{\rm{SSVQE}}}{\theta_i}{x_\mu}\\&=\sum_S\omega^{\rm{VQE}}\pdv{\theta_j}\bra{\psi_j}\hat{U}^\dag(\bm{\theta}^*)\pdv{\hat{\mathcal{H}}(\bm{x},\bm{\kappa}^*)}{x_\mu}\hat{U}(\bm{\theta}^*)\ket{\psi_S}\\
        &\pdv{E^{\rm{SA}}}{\kappa_{pq}}{x_\mu}=\sum_{S}\omega_S^{\rm{SA}}\pdv{\kappa_{pq}}\bra{\psi_S}\hat{U}(\bm{\theta}^*)\pdv{\hat{\mathcal{H}}(\bm{x},\bm{\kappa}^*)}{x_\mu}\hat{U}(\bm{\theta}^*)\ket{\psi_S}.
    \end{split}
\end{equation}

Solving coupled linear equations Eq.\eqref{eq:straightforward linear} gives the derivatives of parameters, and thus yields analytical gradients of the state-specific energy. Note that the number of required additional circuits in this approach is the same as in the Lagrangian method. %In this sense, the Lagrangian method makes no difference in workload of quantum computer.
However, we emphasize that linear equations Eq.\eqref{eq:straightforward linear} have to be calculated for each $x_\mu$ in this approach, which amounts to huge computational cost. We need to solve linear equations Eq.\eqref{eq:matrix vqd} only once in the Lagrangian method, which provides a clear advantage.           
\end{comment}
